The Radio-Loud Fraction of Quasars is a Strong Function of Redshift and Optical Luminosity

Using a sample of optically-selected quasars from the Sloan Digital Sky Survey, we have determined the radio-loud fraction (RLF) of quasars as a function of redshift and optical luminosity. The sample contains more than 30,000 objects and spans a redshift range of 0<z<5 and a luminosity range of -30<M_i<-22. We use both the radio-to-optical flux ratio (R parameter) and radio luminosity to define radio-loud quasars. After breaking the correlation between redshift and luminosity due to the flux-limited nature of the sample, we find that the RLF of quasars decreases with increasing redshift and decreasing luminosity. The relation can be described in the form of log(RLF/(1-RLF)) = b_0 + b_z log(1+z) + b_M (M_{2500}+26), where M_{2500} is the absolute magnitude at rest-frame 2500A, and b_z, b_M<0. When using R>10 to define radio-loud quasars, we find that b_0=-0.132+/-0.116, b_z=-2.052+/-0.261, and b_M=-0.183+/-0.025. The RLF at z=0.5 declines from 24.3% to 5.6% as luminosity decreases from M_{2500}=-26 to M_{2500}=-22, and the RLF at M_{2500}=-26 declines from 24.3% to 4.1% as redshift increases from 0.5 to 3, suggesting that the RLF is a strong function of both redshift and luminosity. We also examine the impact of flux-related selection effects on the RLF determination using a series of tests, and find that the dependence of the RLF on redshift and luminosity is highly likely to be physical, and the selection effects we considered are not responsible for the dependence.

==> response <==
This is a revised paper.

Manuscript #: 65643
Title:  The Radio-Loud Fraction of Quasars is a Strong Function of 
  Redshift and Optical Luminosity
The paper contains:
  ms.tex:                 main tex file
  f1.eps --> f7.eps:      7 eps figures

Name: Linhua Jiang
Address: Steward Observatory, University of Arizona,
         933 North Cherry Avenue, Tucson, AZ 85721
Phone: 520-621-6535
Fax:   520-621-1534
E-mail: ljiang@as.arizona.edu

------------------------------------------------------------
Thanks for Dr. Ari Laor (editor) and the referee's comments.
The following is the response to these comments.

********************
Dr. Laor's comments:

> I have a comment you may want to consider, but please do not feel obligated 
> to refer to it in any way. This may be relevant to understanding the 
> apparent contradiction between the recent White et al. result that the mean 
> R decreases with increasing luminosity, and your result that the fraction of 
> radio loud AGN increases with luminosity (see report below). Looking at Fig.1
> in Xu et al. (1999), one can see there is a bimodal distribution in R at all
> L_[O III], but the "valley" between the two populations is not at a fixed R, 
> but rather the R which separates the two populations decreases with 
> increasing L_[O III] (since L_radio\propto L_[O II]^0.5). This figure shows 
> that the radio loud region becomes more populated, compared to the radio 
> quiet one, as L_[O III] increases, though the mean R at a given L_[O III] 
> may still be going down. I am not sure this will work quantitatively, but 
> you may want to check (see a few more words on that in astro-ph/0312417). 

Re:
Yes, this is an interesting point. It is certainly true that the apparent 
discrepancy between the papers might be explained by a difference between 
the average and extreme properties of the sample as a function of 
luminosity. However, it is difficult to make direct comparison with the 
Xu99 results due to the following reasons. 
1) We are considering optically-selected quasars; while in Xu99, quasars were 
selected as those having both [OIII] emission line and 5 GHz measurements.
This radio selection has bias against radio-quiet quasars. 2) Xu99 uses all 
classes of AGNs, including SyI, SyII, BLRG, NLRG, quasars etc, while we are 
only dealing with broad-line quasars. Xu99 plots their results for quasars 
in Fig 2b, where no trend is obvious, though the valley is still there. 
At logL[OIII]>36, there are no radio-quiet quasars in that figure due to
the sample incompleteness. 3) Xu99 uses a relatively small sample of ~400 
sources (the number of quasars is <200), which were taken from four different 
databases. The incompleteness could cause different effects. They found a 
"very" clear separation between RL and RQ quasars. Though SDSS and FIRST do 
not go very deep, we did not find this clear valley at the bright end.
4) We define R=radio/optical continuum, while Xu99 uses the ratio of radio to 
[OIII]. There is probably no or week correlation between optical continuum and 
[OIII] emission, especially when they use both type 1 and type 2 quasars/AGNs.
Therefore it is hard to make a direct comparison.

************************
Referee's main comments:

> The combination of large area radio and quasar surveys, such as FIRST
> and SDSS, should allow us to finally answer these questions
> definitively. However, upon comparison of this paper and the recent
> paper by White, Helfand, Becker, Glikman \& de Vries,
> astro-ph/0607335, I am left in a rather confused state. The White et
> al. paper uses a stacking procedure which utilises information from
> FIRST-detected and FIRST-undetected SDSS quasars. They find that the
> radio-loudness parameter R* is a NEGATIVE function of optical
> luminosity and that when this luminosity-dependence is removed, there
> is NO dependence on redshift. This is quite at odds with the paper by
> Jiang et al. which claims the RLF is a POSITIVE function of optical
> luminosity and a NEGATIVE function of redshift.

> I have spent much time trying to reconcile these two views and it is
> not easy to do. The RLF and the median R* are not identical and it is
> possible that this explains the differing results. The RLF is the
> fraction of quasars exceeding a threshold in R* and therefore depends
> upon only the behaviour at high values of R*. The median R* is the
> median value of R* and therefore depends only upon the behaviour close
> to the median value which is at low R*. So if one believes the R*
> distribution is bimodal then the RLF result corresponds to the
> behaviour of radio-loud quasars, whereas the median R* result
> corresponds to the behaviour of radio-quiet quasars. If true, this
> would be a very interesting finding of different luminosity and
> evolutionary behaviour for these two classes of quasars.

Re:
We had read White06 and talked to White and Becker before we submitted
the paper. It is difficult to reconcile the two results. As you said,
one explanation is that the RLF and the median R are not identical.
The RLF is the fraction of quasars exceeding a threshold in R, and 
therefore corresponds to the behavior of a small fraction of quasars with
high R (or radio-loud quasars); while median R is dominated by majority
quasars with low R (or radio-quiet quasars). In our paper, radio-loud and
-quiet quasars do not have to be two totally different populations, i.e.,
the distribution of R can be bimodel or continuous.

As we discussed in the last paragraph of sec 5, there are two natural ways 
to interpret the RLF as a function of redshift and luminosity. 1) the 
cosmological evolution of quasar radio properties, such as R and L_r. 
For example, a decreasing R directly results in a decreasing RLF for 
increasing redshift. 2) the density evolution of different populations of 
quasars (e.g. radio-loud and radio-quiet). White06 probably rules out the 
first explanation. Then the 2nd explanation becomes promising. That is, 
at low redshifts there are more RL quasars. But the fraction of RL quasars
is small, so they do not change the median R, which is still dominated by 
radio-quiet quasars. We have included these discussion in the current 
version.

> However, another plausible explanation of the difference is that the
> incompleteness of FIRST has a higher impact on the Jiang et
> al. results than has been considered. It is striking that the RLF
> appears to be such a strong function of i-band magnitude. For the
> k-corrections assumed, the i-band limit of i=18.9 corresponds to R*=10
> at a radio flux density of 1.1 mJy. The authors use 1.1 mJy as their
> FIRST detection limit, but also state that this is the median 5sigma
> flux density limit in FIRST. If this is the median limit, then the
> catalogue is 50% incomplete as this level. This could have a huge
> impact on the RLF because the total change in RLF over luminosity
> and/or redshift is only a factor of two. The authors should make it
> clear if this incompleteness has been accounted for and if not then
> account for it explicitly in their work. The authors do address the
> FIRST incompleteness in Sec.5, but there they calculate how incomplete
> FIRST needs to be to eliminate any dependence of the RLF on luminosity
> and redshift. Since the FIRST incompleteness as a function of flux
> density is well-known, it is better to include this before showing
> results, since it will not completely remove the luminosity and
> redshift dependences, but may weaken them somewhat. 

Re:
The median limit of 0.98 mJy already includes the CLEAN bias correction 
(I did not realize it in the previous version). The FIRST limit is quite 
uniform, and only ~4% of the quasars have limits above 1.1 mJy. Therefore 
we used 1.1 mJy as the limit. Many sources in FIRST images are resolved.
The resolution effect causes FIRST more incomplete for extended objects 
near the detection limit. Furthermore, FR2 quasars are more incomplete
than FR1 quasars for integrated flux densities. White provided us 
the FIRST completeness as a function of integrated flux density.
The completeness is computed using the observed size distribution and rms 
values from the FIRST survey for SDSS quasars, and has included all effects 
mentioned above. This has been shown in Figure 1 in the paper. 
We correct for the sample incompleteness in the current version using this 
completeness curve. 
For a quasar with f_int>5 mJy, its completeness fraction g_comp is roughly
1 (100%); while for a quasar with 1.1 mJy<f_int<5 mJy, its g_comp
is measured from the curve. To correct for the sample incompleteness, we use
the weight of 1/g_comp when we calculate the numbers of radio-loud
quasars. We address this in Sec 3.

We also add two new tests (Tests 6 and 7) in the current version using the 
limit of 1.5 mJy (the corresponding i~18.6) for R>10 and using the limit of 
3 mJy (corresponds to i~18.9) for R>30. The completeness is about 75% at 
1.5 mJy and 95% at 3 mJy. We get the similar results in these tests. 
See the right panel on (for Test 7),
http://quasar.as.arizona.edu/~jiang/radio/test7.eps

Actually the FIRST completeness is not important as we might have thought.
The reason is that we are considering relative numbers, not absolute 
values. FIRST only recognizes 20cm radio emission, and it does not care about 
redshift or optical luminosity. For example, for a given object with a 
"true" observed 20cm flux density of 1mJy, whatever the optical brightness 
is, or whatever the redshift is, FIRST has the same chance to detect it or
miss it, as long as other radio properties do not change with redshift.
For the standard cosmology, the angular distance changes by only 20% for 
0.5<z<4, so the size distribution changes a little with redshift if there
is no physical evolution on radio sizes. In addition, we find that
the physical radio size is also independent of optical luminisotiy,
http://quasar.as.arizona.edu/~jiang/radio/test94.eps
where x axis is absolute magnitude, and y axis is physical radio size
(calculated from major axis in the FIRST catalog).

> Is it possible that White et al. found the wrong dependence of the
> median R* upon luminosity because they did not split the sample up
> into redshift bins? If they had found a steeper correlation with
> luminosity (similar to that of Jiang et al.)  then they would have
> been left with a negative redshift dependence. Their Fig. 10 would
> appear to argue against this where they do show a similar radio
> luminosity - optical magnitude relationship at different redshifts.

Re:
Another explanation for the different results is that White06 did not break
the luminosity-redshift degeneracy. White06 computed the radio luminosity
as a function of the optical luminosity without taking into account
redshift dependence. Then they looked for a dependence of the residuals
from this relationship on redshift. This is not the same thing as
simultaneously computing logL_R as a function of both log(1+z) and logL_opt.
However, this is probably not a good explanation, since White06
found the same trend in small redshift bins.

> I believe the Jiang et al. paper needs to fully address this issue
> before it is acceptable for publication. Inclusion of FIRST
> incompleteness is vital and discussion with the White et al. team
> and some analysis of median stacking may be necessary to fully
> reconcile these two works. I believe the resulting paper will be
> considerably stronger if it can link the differing findings of the
> different methods.

Re:
As we said above, we have added a few paragraphs to address this issue
in the current version. We also added more discussion to try to 
reconcile the two different results.

Other comments:
***************

> 1. It may be worthwhile limiting the whole paper to z<2.2 because
>    beyond this the SDSS selection effects, particularly those
>    associated with colour, begin to dominate. Since these analyses are
>    so dominated by selection effects, the most convincing answer may
>    come from a smaller, but cleaner, sample. Alternatively, it would
>    also be acceptable to have this redshift limit just as a separate
>    figure, as in this version of the paper.

Re:
The SDSS quasar selection at z>2.2 is actually quite complete (e.g. 
Richards et al. 2006), so we do not want to discard these data. In addition, 
x-axes of most plots in our paper are redshift, therefore readers can still 
see RLFs in different redshift ranges, including the range of z<2.2.
Anyway, we made a plot similar to fig 5 for only z<2.2 quasars,
http://quasar.as.arizona.edu/~jiang/radio/fig5b.eps

> 2. Section 5 discusses the results. I felt the comparison with
>    previous small samples was unnecessary since these have large
>    Poisson uncertainties given the low values of the RLF. The final
>    paragraph deals with interpretation of the evolution in RLF, which
>    is the key finding of this paper. This section could be more
>    enlightening given the importance of this result.

Re:
Yes, you are right. We have deleted this paragraph in the current version, 
and also added more discussion in the last paragraph.

> 3. Section 6. The comparison with the optical luminosity function
>    incompleteness that wasn't is not physically related to the
>    similar-looking behaviour of the RLF so is not relevant to this
>    paper.

Re: 
Yes, you are right. We have deleted this paragraph in the current version.

> 4. Put z as well as log (1+z) on x-axes of plots.

Re:
Yes, you are right. We have done this in the current version.

> 5. Fig. 2. Show also a bin for -27.4<M_2500<-26.8 which has quasars
   over a wide redshift range.

Re:
Yes, you are right. We have done this in the current version.

